Distributed Strategies for Dynamic Coverage with Limited Sensing Capabilities

In this work, it is presented the development of a novel distributed algorithm performing robotic coverage, clustering and dispatch around an event in static-obstacle structured environments without relying on metric information. Specifically, the aim is to account for the trade-off between local communication given by bearing visibility sensors installed on each agent involved, optimal deployment in closed unknown scenarios and focus of a group of agents on one point of interest. The particular targets of this study can be summarized as 1. the computation, under certain topological assumptions, of a lower bound for the number of required agents, which are provided by a realistic geometric model (e.g. a round shape) to emphasize physical limitations; 2. the minimization of the number of nodes and links maintaining a distributed approach over a connected communication graph; 3. the identification of an activation cluster around an event with a radial decreasing intensity, sensed by each agent; 4. the attempt to send the agents belonging to the cluster towards the most intense point in the scenario by minimizing a weighted isoperimetric functional.

==> tikzDefs.tex <==
\makeatletter

% Set some defaults 
\tikzset{
    plane max x/.initial=2,
    plane max y/.initial=2,
    plane max z/.initial=2
}

\tikzset{plane/.style={fill opacity=0.5}}

% Define a plane.
% #1 = name of the plane
% #2*x + #3*y + #4*z = #5 is the equation of the plane
\newcommand*\definePlaneByEquation[5]{
    \expandafter\gdef\csname tsx@plane@#1\endcsname{
        \def\tsx@plane@xcoeff{#2}
        \def\tsx@plane@ycoeff{#3}
        \def\tsx@plane@zcoeff{#4}
        \def\tsx@plane@scalar{#5}
    }
}

% Draw a plane.
% The optional first argument is passed as options to TikZ.
% The mandatory second argument is the name of the plane.
\newcommand\drawPlane[2][]{
    \tikzset{plane max x/.get=\tsx@plane@maxx}
    \tikzset{plane max y/.get=\tsx@plane@maxy}
    \tikzset{plane max z/.get=\tsx@plane@maxz}
    \csname tsx@plane@#2\endcsname

    \ifdim\tsx@plane@xcoeff pt=0pt
        \ifdim\tsx@plane@ycoeff pt=0pt
            \ifdim\tsx@plane@zcoeff pt=0pt
                %invalid plane
            \else % x=0, y=0
                \filldraw[plane,#1,shift={(0,0,\tsx@plane@scalar/\tsx@plane@zcoeff)}]
                    (0,0,0) --
                    (\tsx@plane@maxx,0,0) --
                    (\tsx@plane@maxx,\tsx@plane@maxy,0) --
                    (0,\tsx@plane@maxy,0) --
                    cycle;
            \fi
        \else % x=0, y != 0
            \ifdim\tsx@plane@zcoeff pt=0pt % x=0, z=0
                \filldraw[plane,#1,shift={(0,\tsx@plane@scalar/\tsx@plane@ycoeff,0)}]
                    (0,0,0) --
                    (\tsx@plane@maxx,0,0) --
                    (\tsx@plane@maxx,0,\tsx@plane@maxz) --
                    (0,0,\tsx@plane@maxz) --
                    cycle;
            \else % x=0
                \filldraw[plane,#1]
                    (0,\tsx@plane@scalar/\tsx@plane@ycoeff,0) --
                    (0,0,\tsx@plane@scalar/\tsx@plane@zcoeff) --
                    (\tsx@plane@maxx,0,\tsx@plane@scalar/\tsx@plane@zcoeff) --
                    (\tsx@plane@maxx,\tsx@plane@scalar/\tsx@plane@ycoeff,0) --
                    cycle;
            \fi
        \fi
    \else % x!=0
        \ifdim\tsx@plane@ycoeff pt=0pt % x!=0,y=0
            \ifdim\tsx@plane@zcoeff pt=0pt % x!=0,y=0,z=0
                \filldraw[plane,#1,shift={(\tsx@plane@scalar/\tsx@plane@xcoeff,0,0)}]
                    (0,0,0) --
                    (0,0,\tsx@plane@maxz) --
                    (0,\tsx@plane@maxy,\tsx@plane@maxz) --
                    (0,\tsx@plane@maxy,0) --
                    cycle;
            \else % x!=0,y=0,z!=0
                \filldraw[plane,#1]
                    (\tsx@plane@scalar/\tsx@plane@xcoeff,0) --
                    (0,0,\tsx@plane@scalar/\tsx@plane@zcoeff) --
                    (0,\tsx@plane@maxy,\tsx@plane@scalar/\tsx@plane@zcoeff) --
                    (\tsx@plane@scalar/\tsx@plane@xcoeff,\tsx@plane@maxy,0) --
                    cycle;
            \fi
        \else % x!=0,y!=0
            \ifdim\tsx@plane@zcoeff pt=0pt % x!=0,y!=0,z=0
                \filldraw[plane,#1]
                    (\tsx@plane@scalar/\tsx@plane@xcoeff,0) --
                    (0,\tsx@plane@scalar/\tsx@plane@ycoeff,0) --
                    (0,\tsx@plane@scalar/\tsx@plane@ycoeff,\tsx@plane@maxz) --
                    (\tsx@plane@scalar/\tsx@plane@xcoeff,0,\tsx@plane@maxz) --
                    cycle;
            \else % x!=0,y!=0,z!=0
                \filldraw[plane,#1]
                    (\tsx@plane@scalar/\tsx@plane@xcoeff,0,0) --
                    (0,\tsx@plane@scalar/\tsx@plane@ycoeff,0) --
                    (0,0,\tsx@plane@scalar/\tsx@plane@zcoeff) --
                    cycle;
            \fi
        \fi
    \fi
}

% Define a point.
% #1 = name of the point
% (#2,#3,#4) is the location.
% Also creates a coordinate node of name #1 at the location.
\newcommand\definePointByXYZ[4]{
    \coordinate (#1) at (#2,#3,#4);
    \expandafter\gdef\csname tsx@point@#1\endcsname{
        \def\tsx@point@x{#2}
        \def\tsx@point@y{#3}
        \def\tsx@point@z{#4}
    }
}

% Project a point to a plane.
% #1 = name of the new point
% #2 = name of old point
% #3 = name of plane
\newcommand\projectPointToPlane[3]{{
    \csname tsx@point@#2\endcsname
    \csname tsx@plane@#3\endcsname

    % square of norm of the normal vector
    \pgfmathparse{\tsx@plane@xcoeff*\tsx@plane@xcoeff + \tsx@plane@ycoeff*\tsx@plane@ycoeff + \tsx@plane@zcoeff*\tsx@plane@zcoeff}
    \let\nnormsq\pgfmathresult

    % Calculate distance in terms of the (non-normalized) normal vector
    \pgfmathparse{(\tsx@point@x*\tsx@plane@xcoeff + \tsx@point@y*\tsx@plane@ycoeff + \tsx@point@z*\tsx@plane@zcoeff - \tsx@plane@scalar) / \nnormsq}
    \let\distance\pgfmathresult

    % Calculate point
    \pgfmathparse{\tsx@point@x - \distance*\tsx@plane@xcoeff}
    \let\x\pgfmathresult
    \pgfmathparse{\tsx@point@y - \distance*\tsx@plane@ycoeff}
    \let\y\pgfmathresult
    \pgfmathparse{\tsx@point@z - \distance*\tsx@plane@zcoeff}
    \let\z\pgfmathresult

    \definePointByXYZ{#1}{\x}{\y}{\z}
}}
\makeatother

